The Chemical Nature of the Young 120-Myr-old Nearby Pisces-Eridanus Stellar Stream Flowing through the Galactic Disk

Recently, a new cylindrical-shaped stream of stars up to 700 pc long was discovered hiding in the Galactic disk using kinematic data enabled by the Gaia mission. This stream of stars, dubbed Pisces-Eridanus (Psc-Eri), was initially thought to be as old as 1 Gyr, yet its stars shared a rotation period distribution consistent with a population that was 120-Myr-old. Here, we explore the detailed chemical nature of this stellar stream. We carried out high-resolution spectroscopic follow-up of 42 Psc-Eri stars using McDonald Observatory, and combined these data with information for 40 members observed with the low-resolution LAMOST spectroscopic survey. Together, these data enabled us to measure the abundance distribution of light/odd-Z (Li, Na, Al, Sc, V), $\alpha$ (Mg, Si, Ca, Ti), Fe-peak (Cr, Mn, Fe, Co, Ni, Zn), and neutron capture (Sr, Y, Zr, Ba, La, Nd, Eu) elements along the Psc-Eri stream. We find that the stream is (1) near solar metallicity with [Fe/H] = -0.03~dex and (2) has a metallicity spread of 0.07~dex (or 0.04 dex when outliers are excluded). We also find that (3) the abundance of Li indicates that Psc-Eri is $\sim$120 Myr old, consistent with its gyrochronology age. Additionally, Psc-Eri has (4) [X/Fe] abundance spreads which are just larger than the typical uncertainty in most elements, (5) it is a cylindrical-like system whose outer edges rotate about the center and, (6) no significant abundance gradients along its major axis except a potentially weak gradient in [Si/Fe]. These results show that Psc-Eri is a uniquely close, young, chemically interesting laboratory for testing our understanding of star and planet formation.

==> commands.tex <==
% Seismology shortcuts
\newcommand{\numax}{\mbox{$\nu_{\rm max}$}\xspace}
\newcommand{\dnu}{\mbox{$\Delta \nu$}\xspace}
\newcommand{\teff}{\mbox{$T_{\rm eff}$}\xspace}
\newcommand{\logg}{\mbox{$\log g$}\xspace}
\newcommand{\feh}{\mbox{$\rm{[Fe/H]}$}\xspace}
\newcommand{\msun}{\mbox{$\mathrm{M}_{\odot}$}\xspace}
\newcommand{\lsun}{\mbox{$\mathrm{L}_{\odot}$}\xspace}
\newcommand{\mearth}{\mbox{$\mathrm{M}_{\oplus}$}\xspace}
\newcommand{\rsun}{\mbox{$\mathrm{R}_{\odot}$}\xspace}

% Hall+19 shortcuts
\newcommand{\oozp}{\mbox{$\varpi_{\rm zp}$}\xspace}
\newcommand{\muas}{\mbox{$\mu \rm as$}\xspace}
\newcommand{\murc}{\mbox{$\mu_{\rm RC}$}\xspace}
\newcommand{\fdnu}{\mbox{$f_{\Delta\nu}$}\xspace}
\newcommand{\sigrc}{\mbox{$\sigma_{\rm RC}$}\xspace}

% Maths
\newcommand{\logten}{\mbox{$\log_{10}$}\xspace}

% Units
\newcommand{\muHz}{\mbox{$\mu$Hz}\xspace}
\newcommand{\Ks}{\mbox{$K$}\xspace}
\newcommand{\kms}{\,km\,s$^{-1}$\xspace} % kilometres per second

% Other
\newcommand{\kepler}{\emph{Kepler}\xspace}
\newcommand{\hipparcos}{\emph{Hipparcos}\xspace}
\newcommand{\ktwo}{\emph{K2}\xspace}
\newcommand{\gaia}{\emph{Gaia}\xspace}
\newcommand{\bibtex}{\textsc{Bib}\!\TeX} % bibtex. Not quite the correct typesetting, but close enough

